Analysis and controller-design of time-delay systems using TDS-CONTROL. A tutorial and manual

TDS-CONTROL is an integrated MATLAB package for the analysis and controller-design of linear time-invariant (LTI) dynamical systems with (multiple) discrete delays, supporting both systems of retarded and neutral type. TDS-CONTROL is based on a state-space representations for these TDSs, although functionality is provided to obtain such a formulation from a frequency-domain description of the system. Firstly, the package offers various functionality for analyzing such systems, like methods for computing the spectral abscissa, the H-infinity norm, the pseudospectral abscissa, and the distance to instability. Furthermore, as TDS-CONTROL is designed with neutral time-delay systems in mind, it has the appealing feature that the sensitivity of certain quantities (such as the spectral abscissa) with respect to infinitesimal delay perturbations can explicitly be taken into account. Secondly, TDS-CONTROL also allows to design fixed-order dynamic output feedback controllers. The corresponding controller-design algorithms are based on minimizing the spectral abscissa, the H-infinity norm, or a combination of both with respect to the free controller parameters by solving a non-smooth, non-convex optimization problem. As a strictly negative spectral abscissa is a necessary and sufficient condition for stability, the presented design methods are thus not conservative. It is also possible to impose structure on the controller, enabling the design of decentralized and proportional-integral-derivative (PID) controllers. Furthermore, by allowing the plant to be described in delay descriptor form (i.e., the system's dynamics are given in terms of delay differential algebraic equations), acceleration feedback and Pyragas-type and delay-based controllers can also be considered.

==> chapters/documentation/tds_create.tex <==
% !TeX root = ../../main.tex
\section{\texorpdfstring{\texttt{tds\_create}}{tds\_create}, \texorpdfstring{\texttt{tds\_create\_neutral}}{tds\_create\_neutral}, and \texorpdfstring{\texttt{tds\_create\_ddae}}{tds\_create\_ddae}}
The functions \texttt{tds\_create}, \texttt{tds\_create\_neutral}, and \texttt{tds\_create\_ddae} create a \matlabfun{tds} representation for respectively a retarded time-delay system, a neutral time-delay system or a delay descriptor system. Below we w\\

\subsection{Examples}
Retarded delay differential equation
\[
\dot{x}(t) = 
\]
\begin{lst}
	inhoud...
\end{lst}
